Fundamental Diagrams of Commercial Adaptive Cruise Control: Worldwide Experimental Evidence

Experimental measurements on commercial adaptive cruise control (ACC) vehicles \RoundTwo{are} becoming increasingly available from around the world, providing an unprecedented opportunity to study the traffic flow characteristics that arise from this technology. This paper adds new experimental evidence to this knowledge base and presents a comprehensive empirical study on the ACC equilibrium behaviors via the resulting fundamental diagrams. We find that like human-driven vehicles, ACC systems display a linear equilibrium spacing-speed relationship (within the range of available data) but the key parameters of these relationships can differ significantly from human-driven traffic depending on input settings: At the minimum headway setting, equilibrium capacities in excess of 3500 vehicles per hour are observed, together with an extremely fast equilibrium wave speed of 100 kilometers per hour on average. These fast waves are unfamiliar to human drivers, and may pose a safety risk. The results also suggest that ACC jam spacing can be much larger than in human traffic, which reduces the network storage capacity.

==> sections/old/5_FD.tex <==

% \todo[inline]{look until here}
% \todo[inline]{to do,  change our name to M1-4. compare our results with Dan's results}

\section{\textbf{Characteristics of ACC $s-v$ relationships and the fundamental diagrams}}
In this section, we translate the $s-v$ relationships to the fundamental diagrams (FDs) that connect the flow, density, and speed from the macroscopic perspective.  We further investigate the characteristics of the $s-v$ relationships and the FDs; i.e. capacity, wave speed, and jam spacing.

In our analysis, we consolidate the data across the four experiments to obtain a more comprehensive coverage of the  $s-v$ relationships whenever possible.  Specifically, some car models were tested in more than one experiments. In that case, we conduct a statistical test on the estimated $s-v$ relationships from different data sources and combine them only if the estimated results are statistically insignificant. We find that the estimated $s-v$ relationships from different experiments are consistent, except for one case - one car model estimated from AstaZero differed from the estimations from MA experiment and ZalaZone.  That is likely because the measurement systems have different measurement errors (more discussions on this will follow in Session \ref{spacing_variation}).  Nevertheless, for this case, we have excluded the data from AstaZero and combine the data from the other two sources.   

% \todo[inline]{
% 1. a typical ACC sv, qk;
% 2. Dan’s 7 Toyota have mid-range: 15-30m/s
% Tesla S has low –high speed: 7-30m/s
% Tesla 3 has low –high speed: 7-30m/s
% Several car models tested in Zalazone only have low-medium speed: 7-15m/s
% 3. dist of tau and delta
% 4. all sv, all qk
% - capacity, jam density
% 5. discussion (spacing variance)
% }



\subsection{\textbf{Typical $s-v$ features}}


% - linear is good
% - seems one relationship for a wide range
% - in most speed ranges, ACC is within HDV boundaries.  But it falls outside in two regions.  (1) high speed in min, it's below the lower bound, resulting in higher capacity than HDV uppper bound.  (2) low speed in min and max (?), it's above the HDV UB, suggesting smaller flow in extremely low speed (close to stop).  Of course,  such extremely low speed condition was not tested.  Need further research.  This is likely if the excessive spacing is smaller than a vehicle length. E.g., in Tesla S min, 

\subsubsection{\textbf{A typical $s-v$ relationship}}
Figure \ref{sv_qk_single} (a) shows the estimated $s-v$ relationships of one evaluated ACC system (system H). One can see that the ACC equilibrium points are well aligned on the linear curve in both headway settings. The linear relationship also holds in a wide speed range. In the plot (and other $s-v$ plots later), we also provide the references from HDVs (red dashed line for the mean , and orange dotted lines for the 15th and 85th percentiles, denoted as $P_{15}$ and $P_{85}$, representing HDV bounds) taken from \cite{chen2012behavioral} that measured $\tau_0$ and $\delta_0$ of individual drivers in the NGSIM dataset \citep{NGSIM_2006}. Note that, the variation of $\tau_0$ and $\delta_0$ in HDVs \citep{chen2012behavioral} stems from the difference of individual HDVs, which is a holistic outcome of the heterogeneity from drivers and the vehicles used, thus is different from this study.  Nevertheless, their distributions provide some references of the HDVs. 

Based on an estimated $s-v$ relationship, we can estimate the corresponding $q-k$ relationship (i.e., the fundamental diagram); see Figure \ref{sv_qk_single}(b).  Specifically, a linear $s-v$ relationship translates to a triangular shaped fundamental diagram; i.e.,  $w= -\delta_0/\tau_0$, $k_j= 1/\delta_0$, and $Cap = u_f / (u_f \tau_0 + \delta_0) =- k_j w u_f/(u_f-w)$. Note that the capacity depends on free-flow speed $u_f$. Here we project the capacity at $u_f=105km/h$ $(65mph)$ as it is near the higher bound of the ACC systems tested. 

It is found that the ACC system is very different from HDV, especially in minimum headway, in most speed levels. The H-max $s-v$ line is mostly above the HDV mean, but still inside the HDV bounds. Notably, the H-min $s-v$ line falls outside the HDV bounds in two regions: (i) in mid-high speed levels (larger than \SI{12}{m/s}), the ACC  spacing is smaller than HDV lower bound (see Figure \ref{sv_qk_single} (a)), suggesting a much higher capacity than HDV higher bound (see Figure \ref{sv_qk_single}(b)); (ii) in very low speed (close to stop), the ACC spacing is above the HDV upper bound, suggesting smaller jam density. Moreover, one can see from Figure \ref{sv_qk_single}(b) that H-min embeds a very fast propagating wave speed (\SI{-70.7}{km/h}) that is vert different from HDV.
Nevertheless, it should be noted that for most of the car models examined in the literature, the very low speed condition (i.e., near jam density) was not tested and the extrapolation may not represent the real conditions. More studies along this line will follow. 
% \todo{not sure whether this still holds.  Check the 15 and 85 percentile.  Need to update this whole paragraph}
% , with the H-min  $s-v$ line mostly below the HDV mean and H-max  $s-v$ line above the HDV mean.  
% Notably, it falls outside the HDV bounds in two regions: (i) high speed at the minimum headway setting, where the ACC spacing can go below the HDV lower bound (see Figure \ref{sv_qk_single} (a)), suggesting a higher capacity than HDV upper bound (see Figure \ref{sv_qk_single}(b)); (ii) very low speed (close to stop) at the minimum headway setting, where the ACC spacing is above the HDV upper bound, suggesting smaller jam density. Nevertheless, it should be noted that for most of the car models examined in the literature, the very low speed condition was not tested and the extrapolation may not represent the real conditions.  More discussion along this line will follow. 

% \hl{Need to update this based on the 15 and 85 percentile HDV}

% \todo[inline]{comment on 
% - s-v relationship compared to HDV
% - capacity
% - wave speed, jam density}




% \hl{ to add qk estimation? The $s-v$ translates to a triangular shape $q-k$ plot.  add}. 

% Moreover, two worthnoting features of the data used in this paper are observed: (i) We do not have full speed coverage on the equilibrium data. The minimum observed equilibrium speed is about \SI{15}{m/s} here for the system Y. Additionally, the equilibrium cases are clustered in several narrow speed bins. (ii) Significant speed variation are observed in each speed bin. Even for the same ACC system with the same setting, the equilibrium spacing can vary largely in a small speed range, i.e., though a general linear $s-v$ relationship is found,  the ACC controller does not strictly hold it.

% Here, feature (i) relates to the the design of the experiments which is the limitation of our analyzed data, while feature (ii) reveals interesting characteristics of the ACC controller itself. We thereafter discuss them respectively.

\noindent
\begin{minipage}{\linewidth}
\centering
\begin{minipage}[b]{.49\linewidth}
\centering
\small
\includegraphics[height=175pt]{figures/s-v single.png}
\\[-6pt]
(a) $s-v$ relationship
\end{minipage}
\begin{minipage}[b]{.49\linewidth}
\centering
\small
\includegraphics[height=175pt]{figures/q-k single.png}
\\[-6pt]
(b) $q-k$ relationship
\end{minipage} 
\captionof{figure}{FD of ACC system H}
\label{sv_qk_single}
\end{minipage}

% We have consolidated the four data sources to estimate the $s-v$ relationships for each car model and the detailed results are provided in Appendix Table \ref{full_sv_regression_table}. 
%Figure \ref{speed_range} shows the speed range of observed equilibrium cases for the tested car models. The grey bar indicates the overall observed range of the car, and the red slots indicate the speed bins with observed equilibrium cases. Clearly, the equilibrium cases only cover a set of discrete speed levels as the experiments were designed for different purposes. More importantly, most of the ACC systems only have a partial coverage of the speed range.
% Specifically, the data sources will be consolidated if the estimated  $s-v$ relationships are consistent (i.e., statistically insignificant).  Also note that, we require that there are equilibrium data for three or more speed bins from the same data source in order to estimate the $s-v$ relationship for an ACC system. 

% Figure \ref{sv_Manufacturer} shows the $s-v$ relationships of the manufacturers 1, 2 and Tesla using the consolidated data. Results of other manufacturers are in Appendix in Figure \ref{sv_Manufacturer_other}. One can see that in general, linearity yields good approximation for the tested speed ranges.  Particularly, four ACC systems (system D/H/W/X) have a large speed coverage (ranging from \SI{7}{m/s}-\SI{30}{m/s}) after the consolidation, suggesting a good confidence in our estimation. %\todo{do we provide the plots? where?} 
% %\todo{Is it correct?}
% % It is found different manufacturers show some different features, especially for the ones that have multiple car models tested. 

% % For example, for Manufacturer 1 (see Figure \ref{sv_Manufacturer}(a)), the four systems have similar $s-v$ relationships. Figure \ref{sv_Manufacturer}(b) shows obvious difference in minimum headway; i.e., system E has a much larger spacing than system F/G. 
% % For Figure \ref{sv_Manufacturer}(c), spacing of the three systems is very different in maximum headway (X $>$ H $>$ W), while the differences are mostly observable in minimum headway at lower speed  ($< 20m/s$), where system X has larger spacing than system W/H. 
% % Notably, one can see the spacing variation under the same speed could be significant in many cases. %such as Figure \ref{sv_Manufacturer}(d) in which the variance even overshadows the difference of mean between the systems. 
% % We will investigate this in details in Section \ref{spacing_variation}. 

% % \todo[inline]{put the consolidated s-v and qk for each manufacturers here.  Add some descriptions of the features of each manufacture too. }
% % \todo[inline]{put \label{s-v_M2,3} here}

% % \todo{only show (a-c) here. Put the others in the appendix}
% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer1.png}
% \\[-2pt]
% (a) Manufacture 1
% \end{minipage} 
% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer2.png}
% \\[-2pt]
% (b) Manufacture 2
% \end{minipage}
% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer3.png}
% \\[-2pt]
% (c) Manufacture 3
% \end{minipage}

% % \begin{minipage}[b]{.325\linewidth}
% % \centering
% % \footnotesize
% % \includegraphics[width=\textwidth]{figures/manufacturer4.png}
% % \\[-2pt]
% % (d) Manufacture 4
% % \end{minipage} 
% % \begin{minipage}[b]{.325\linewidth}
% % \centering
% % \footnotesize
% % \includegraphics[width=\textwidth]{figures/manufacturer_Tesla.png}
% % \\[-2pt]
% % (e) Tesla
% % \end{minipage} 
% % \begin{minipage}[b]{.325\linewidth}
% % \centering
% % \footnotesize
% % \includegraphics[width=\textwidth]{figures/manufacturer_BMW.png}
% % \\[-2pt]
% % (f) BMW
% % \end{minipage} 

% % \begin{minipage}[b]{.325\linewidth}
% % \centering
% % \footnotesize
% % \includegraphics[width=\textwidth]{figures/manufacturer_audi.png}
% % \\[-2pt]
% % (g) Audi
% % \end{minipage} 
% % \begin{minipage}[b]{.325\linewidth}
% % \centering
% % \footnotesize
% % \includegraphics[width=\textwidth]{figures/manufacturer_Mercedes.png}
% % \\[-2pt]
% % (h) Mercedes
% % \end{minipage} 
% % \begin{minipage}[b]{.325\linewidth}
% % \centering
% % \footnotesize
% % \includegraphics[width=\textwidth]{figures/manufacturer_jaguar.png}
% % \\[-2pt]
% % (i) Jaguar
% % \end{minipage} 
% \captionof{figure}{$s-v$ relationships from the consolidated data}\label{sv_Manufacturer}
% \end{minipage}


Notably, since all car models were not tested in the very low speed range, it's unclear whether the estimated $s-v$ relationships still hold outside the tested ranges.  Fortunately, the GA experiment has collected some jam spacing data for ACC System X (measured when the ACC car was at complete stop). Figure \ref{GA_stopping_distance} demonstrates that $\delta_0$ distributes in the range of \SI{7.7}{m} to \SI{11.56}{m} with the mean \SI{9.86}{m}.  Interestingly, this is larger than the jam spacing of HDVs; see Figure \ref{NGSIM_qk} for one direct measurement using NGSIM data, which yields $\delta_0$ at about \SI{7}{m} (corresponding to $k_j=$\SI{142}{veh/km}). %\todo{we can ask Jorge to add one fig on this} 
Moreover, the measured $\delta_0$ is smaller than the projection from the $s-v$ relationship estimated for low to high speeds (\SI{9.86}{m} vs. \SI{15.00}{m}); see Figure \ref{SystemX_consolidated}.  
In fact, for the GA experiment data, if the stopping condition is excluded, it yields a $s-v$ estimation consistent with the MA and OpenACC experiments, although the tested speed ranges differ; see Figure \ref{SystemX_different_sources}(a). However, it differs ($\tau_0$ larger and $\delta_0$ smaller) if the data from stopping condition is included; see Figure \ref{SystemX_different_sources}(b). 

% Figure \ref{SystemX_consolidated} demonstrates an example of consolidation (system X, minimum headway) with data from different sources. From Figure \ref{SystemX_consolidated}(a), one can see that, while the tested speed ranges differ, %(MA: \SI{}{m/s}, OpenACC: \SI{}{m/s}, GA: \SI{}{})
% , the $s-v$ relationships are generally consistent (statistically insignificant), which yield a good consolidated $s-v$ estimation; see Figure \ref{SystemX_consolidated}(b).  Note that the extrapolation yields a jam spacing of  $\delta_0=15.0m$, which seems much larger than HDVs.  In fact, this observation holds for many ACC systems under the minimum headway settings or even the maximum headway setting (see later in Figure \ref{tau0_vs_delta0}).  Luckily, the GA experiments have collected some jam spacing data for ACC System X (measured when the ACC car was at complete stop).  One can see that $\delta_0$ distributes in the range of \SI{7.7}{m} to \SI{11.56}{m} with the mean \SI{9.86}{m} (Figure \ref{GA_stopping_distance}(a)).  Interestingly, this is larger than the jam spacing of HDVs; see \hl{Figure XX for one direct measurement using NGSIM data, which yields $\delta_0$ about xxx.} \todo{we can ask Jorge to add one fig on this} Also note that, 
% % This raises two interesting issues: (i) the empirical measurement of $\delta_0$ confirms that the jam spacing of ACC System X is larger than the jam spacing of HDVs; see \hl{Figure XX for one direct measurement using NGSIM data, which yields $\delta_0$ about xxx.} \todo{we can ask Jorge to add one fig on this}   (ii) 
% the measured $\delta_0$ is smaller than the projection from the $s-v$ relationship estimated for low to high speeds (\SI{9.86}{m} vs. \SI{15.00}{m}).  In fact, if all the GA experiment data including the stopping condition was used, the estimated $s-v$ relationship differs significantly from the MA and OpenACC experiments, with   the estimated $\tau_0$ much larger and $\delta_0$ much smaller; see Figure \ref{GA_stopping_distance}(b).  


Based on these results, we conjecture that the $s-v$ relationship for system X is not a single linear relationship for the whole speed range.  Instead, it might be piece-wise linear for different speed ranges, or one non-linear relationship but linearity is a good approximation in the tested speed range.  Out of such concerns, in our estimation of the $s-v$ relationship in Figure \ref{SystemX_consolidated} , we only use the low-high speed data and exclude the stopping conditions.  Of course, further research on the very low speed condition (0-\SI{5}{m/s}) is desired to test our hypothesis and complete the $s-v$ relationship. 

\noindent
\begin{minipage}{\linewidth}
\centering
\begin{minipage}[b]{.49\linewidth}
\centering
\small
\includegraphics[height=115pt]{figures/GA_stopping_dist.png}
\end{minipage} 
\captionof{figure}{Spacing distribution of the stopping points in GA experiments}
\label{GA_stopping_distance}
\end{minipage}


\noindent
\begin{minipage}{\linewidth}
\centering
\small
\includegraphics[height=115pt]{figures/qk_measurement_NGSIM.png}
\captionof{figure}{Direct HDV measurement from NGSIM data \citep{laval2011hysteresis}}
\label{NGSIM_qk}
\end{minipage}




\noindent
\begin{minipage}{\linewidth}
\centering
\begin{minipage}[b]{.49\linewidth}
\centering
\small
\includegraphics[height=150pt]{figures/GA.png}
\\[-6pt]
(a) excluding stopping points
\end{minipage}
\begin{minipage}[b]{.49\linewidth}
\centering
\small
\includegraphics[height=150pt]{figures/GA_all_speed.png}
\\[-6pt]
(b) including stopping points
\end{minipage}
\captionof{figure}{Estimated $s-v$ relationships of the GA data}
\label{SystemX_different_sources}
\end{minipage}




\noindent
\begin{minipage}{\linewidth}
\centering
% \begin{minipage}[b]{.49\linewidth}
% \centering
% \small
% \includegraphics[height=150pt]{figures/GA.png}
% \\[-6pt]
% (a) estimated $s-v$ relationships from three sources
% \end{minipage}
\begin{minipage}[b]{.49\linewidth}
\centering
\small
\includegraphics[height=150pt]{figures/GA_consolidated.png}
% \\[-6pt]
% (b) estimated $s-v$ relationship from the consolidated data
\end{minipage} 
\captionof{figure}{Consolidated data and estimated $s-v$ relationship of system X}
\label{SystemX_consolidated}
\end{minipage}



Figure \ref{sv_Manufacturer} shows the $s-v$ relationships of the manufacturers 1, 2 and Tesla using the consolidated data. Results of other manufacturers are in Appendix in Figure \ref{sv_Manufacturer_other}. One can see that in general, linearity yields good approximation for the tested speed ranges.  Particularly, four ACC systems (system D/H/W/X) have a large speed coverage (ranging from \SI{7}{m/s}-\SI{30}{m/s}) after the consolidation, suggesting a good confidence in our estimation. %\todo{do we provide the plots? where?} 
%\todo{Is it correct?}
% It is found different manufacturers show some different features, especially for the ones that have multiple car models tested. 

% For example, for Manufacturer 1 (see Figure \ref{sv_Manufacturer}(a)), the four systems have similar $s-v$ relationships. Figure \ref{sv_Manufacturer}(b) shows obvious difference in minimum headway; i.e., system E has a much larger spacing than system F/G. 
% For Figure \ref{sv_Manufacturer}(c), spacing of the three systems is very different in maximum headway (X $>$ H $>$ W), while the differences are mostly observable in minimum headway at lower speed  ($< 20m/s$), where system X has larger spacing than system W/H. 
% Notably, one can see the spacing variation under the same speed could be significant in many cases. %such as Figure \ref{sv_Manufacturer}(d) in which the variance even overshadows the difference of mean between the systems. 
% We will investigate this in details in Section \ref{spacing_variation}. 

% \todo[inline]{put the consolidated s-v and qk for each manufacturers here.  Add some descriptions of the features of each manufacture too. }
% \todo[inline]{put \label{s-v_M2,3} here}

% \todo{only show (a-c) here. Put the others in the appendix}
\noindent
\begin{minipage}{\linewidth}
\centering
\begin{minipage}[b]{.325\linewidth}
\centering
\footnotesize
\includegraphics[width=\textwidth]{figures/manufacturer1.png}
\\[-2pt]
(a) Manufacture 1
\end{minipage} 
\begin{minipage}[b]{.325\linewidth}
\centering
\footnotesize
\includegraphics[width=\textwidth]{figures/manufacturer2.png}
\\[-2pt]
(b) Manufacture 2
\end{minipage}
\begin{minipage}[b]{.325\linewidth}
\centering
\footnotesize
\includegraphics[width=\textwidth]{figures/manufacturer3.png}
\\[-2pt]
(c) Manufacture 3
\end{minipage}

% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer4.png}
% \\[-2pt]
% (d) Manufacture 4
% \end{minipage} 
% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer_Tesla.png}
% \\[-2pt]
% (e) Tesla
% \end{minipage} 
% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer_BMW.png}
% \\[-2pt]
% (f) BMW
% \end{minipage} 

% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer_audi.png}
% \\[-2pt]
% (g) Audi
% \end{minipage} 
% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer_Mercedes.png}
% \\[-2pt]
% (h) Mercedes
% \end{minipage} 
% \begin{minipage}[b]{.325\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/manufacturer_jaguar.png}
% \\[-2pt]
% (i) Jaguar
% \end{minipage} 
\captionof{figure}{$s-v$ relationships from the consolidated data}\label{sv_Manufacturer}
\end{minipage}

% \todo{switch (a) and (b) here}




% It is worth noting that the equilibrium points at stopping (i.e., speed is zero) in the GA experiments were not included in the above Figure \ref{SystemX_consolidated}. We actually find they potentially do not follow the same $s-v$ relationships with the high-speed points (larger than \SI{7}{m/s}).  Figure \ref{GA_stopping_distance}(a) shows the estimated $s-v$ relationship for the GA experiments with the stopping points included. Apparently, the estimated $s-v$ relationship changes with the additional stopping points  ($\tau_0$ increases and $\delta_0$ decreases). The test results suggest the $s-v$ based on GA data (with the stopping points) are significantly different from the other twos. Figure \ref{GA_stopping_distance}(b) shows the distribution of stopping spacing from the GA experiments. The mean stopping spacing is obviously smaller than the estimated $\delta_0$ using only high-speed data (\SI{9.86}{m} vs. \SI{15.00}{m}). Based on the observation, only the high-speed data points are used for the consolidation and estimating the general $s-v$ relationship of system X. Nevertheless, the difference of $s-v$ relationship indicate that potential piece-wise linearity or non-linearity exist in the controller, which requires further exploration. It should also be cautious that the $\delta_0$ estimation with only high-speed data points does not necessarily equal to the the actual stopping distance.




% .  \hl{to add the Tesla description, discussion about the consolidation, different results from either including the stopping points or not}.  

% \todo[inline]{
% - Consolidated Tesla.  One linear? 
% }

% \todo[inline]{
% - FD implication
% }



% For example, a car system may have piece-wise linear $s-v$ relationships for different speed ranges. It's also possible that the true $s-v$ relationship is non-linear but linear is a good approximation in the tested speed range.  Further research along this line is needed. 




% Figure \ref{speed_range} shows the speed range of observed equilibrium cases for the tested car models. The grey bar indicates the overall observed range of the car, and the red slots indicate the speed bins with observed equilibrium cases. Clearly, the equilibrium cases only cover a set of discrete speed levels as the experiments were designed for different purposes.  
% , i.e., the $s-v$ relationship is always not continually observed for the tested ACC systems. This is because the three experiments are all designed with several stable speed levels, where equilibrium only occurs around them. 

%  More importantly, even counting the lowest and highest bound, the observed speed range is still limited. This features also defer by the design of each experiment set. For example, the ZalaZone set in the OpenACC experiments focuses on the low to medium speed level, therefore the observed equilibrium cases are mostly under \SI{15}{m/s}. The other three sets, on the other hand, mainly tested medium to high speed scenarios thus the equilibrium is mostly found above \SI{15}{m/s}.
 

% {\color{blue} 

%  Figure \ref{speed_range_diff} shows two examples of the $s-v$ estimation, one with a larger speed coverage and more bins (H-min) and the other with smaller speed coverage and limited bins (Rav4-max). Apparently, the regression results with H-min seem describing a more complete picture of the ACC system as more cases are tested. Nevertheless, we still include the estimation results for the systems with smaller speed coverage. We believe the results will still hold as long as a general linear $s-v$ exists along different speed (which is found mostly true from the observed range).
%  We do caution that, if the controller is not linear (e.g., following a piece-wise manner), the estimation results might not hold outside the observed speed range. %Particularly, for the jam spacing when speed is close to \SI{0}{m/s}, where literature has suggested that controller designer can use a different control logic at the very low speed.
 
%  }
 
% %%% I think we don't need these figs.

% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \begin{minipage}[b]{.49\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=.6\textwidth]{figures/h-max.png}
% \\[-2pt]
% (a) System H maximum headway (Work experiments)
% \end{minipage}
% \begin{minipage}[b]{.49\linewidth}
% \footnotesize
% \includegraphics[width=.6\textwidth]{figures/rav4-max.png}
% \\[-2pt]
% (b) Toyota Rav4 maximum headway (OpenACC experiments)
% \end{minipage} 
% \captionof{figure}{$s-v$ estimation results with larger speed coverage and smaller speed coverage}
% \label{speed_range_diff}
% \end{minipage}




\subsubsection{\textbf{ACC $\tau_0$ and $\delta_0$ distributions}}
%

% \subsection{\textbf{Spacing-speed characteristics of the ACC Pool}}
% We have estimated the $s-v$ relationships for all ACC systems evaluated based on the consolidated data; see Appendix Table \ref{full_sv_regression_table}.  
In general, our observations above pertaining to System X hold for all evaluated ACC systems based on the consolidated data.  
Overall,  a linear estimation yields a very good fit ($R^2$ is mostly above 0.8) for most of the models in the tested speed ranges, which usually covers medium to high speeds or even low to high speeds.  %Moreover, the $s-v$ plot is usually below the HDV average under minimum headway but above for maximum headway.   
%However, we emphasize that, the estimation may not hold for speeds outside the tested range. Particularly, the very low speed conditions (usually below \SI{8}{m/s}) may have another $s-v$ relationship, different from the medium-high speeds.   
Figure \ref{time-gap-jam-spacing_dist} shows the estimated $\tau_0$ and $\delta_0$ distribution of the ACC pool examined compared to the reference - HDVs. One can see that, the distribution of $\tau_0$ ($\delta_0$) for ACC exhibits two clusters, representing the lower and upper bounds of the systems evaluated, corresponding to the minimum and maximum headway settings. 
%Moreover, compared to HDVs, the mean of $\tau_0$ in the ACC systems is smaller (\SI{1.38}{s} vs. \SI{1.51}{s}), and
Notice that the $\tau_0$ of the ACC systems is distributed in a much larger range and has a much smaller lower bound (\SI{0.54}{s} vs. \SI{0.91}{s}).  In fact, 65\% of the car models in minimum headway have $\tau_0$ smaller than HDV lower bound.  Regarding $\delta_0$, the ACC pool is distributed in a much wider range and has a much larger upper bound than HDVs (\SI{17.44}{m} vs. \SI{10.74}{m}). Over 56\% of the car models has $\delta_0$ beyond the HDV upper bound .   %As expected, ACC has a larger mean for $\delta_0$ (\SI{10.88}{m} vs. \SI{7.09}{m}).  

%Note that since the experiments involved mostly the minimum and maximum headway settings (except for three in headway-3), the distribution of ACC parameters is not continuous and thus the mean does not necessarily capture the \textit{actual} mean across different headway settings (rather, the mean represents the case when the parameter for a given system is evenly distributed between the minimum and maximum headway). But that still provides a reference for the ACC pool.  

% \todo{put the table in the appendix}


\noindent
\begin{minipage}{\linewidth}
\centering
\begin{minipage}[b]{.49\linewidth}
\centering
\footnotesize
\includegraphics[width=.9\textwidth]{figures/time-gap_dist.png}
\\[-6pt]
(a)
\end{minipage}
\begin{minipage}[b]{.49\linewidth}
\centering
\footnotesize
\includegraphics[width=.9\textwidth]{figures/jam-spacing_dist.png}
\\[-6pt]
(b)
\end{minipage} 
\captionof{figure}{$\tau_0$ and $\delta_0$ distribution of the evaluated ACC systems}\label{time-gap-jam-spacing_dist}
\end{minipage}

Figure \ref{tau0_vs_delta0} shows the $\tau_0$ and corresponding $\delta_0$ across the various ACC systems.  In the minimum headway setting $\delta_0$ is usually larger if $\tau_0$ is smaller; see the circle markers and the orange dash line (p-value = 0.00).  This is expected as a larger $\delta_0$ can compensate the effect of a smaller $\tau_0$ to increase spacing and thus improve safety, which is particularly critical under the minimum headway setting.   One can see that $\tau_0$ is usually quite small (mostly below \SI{1}{s}) and the $\delta_0$ is large, which is mostly above \SI{10}{m} and can reach \SI{18}{m}.  This is very different from HDVs. For the maximum headway, the decreasing trend is not significant (see triangle markers).
% the decreasing trend is not as significant (p-value = 0.06) and the slope is much flatter (see triangle markers and green dashed line).  
This is probably because under the maximum headway, the $\tau_0$ values are generally large and thus safety is not as concerning.  In the maximum headway, the $\delta_0$ is mostly larger than the HDV average with the data points falling in quadrant I.  Interestingly, some systems have a very large $\delta_0$ even though the $\tau_0$ is already large (see those in the upper right of quadrant I), suggesting that the spacing is profoundly larger than HDVs.  \hl{The slope of each point with respect to the origin ($\tau_0=0$, $\delta_0=0$) represents the value of the wave speed $w$.}  

Of course, we again caution that, in all the car models examined here,  except for car model X, $\delta_0$ is the extrapolated outcome, not the direct measurement.  Interestingly, our estimated $\tau_0$ and $\delta_0$ values are actually consistent with the result in \cite{gunter2020commercially} that used another method (more discussion will follow in Section \ref{method_comparison_to_Dans}).  This validates our observations pertaining to $\tau_0$ and $\delta_0$.  

Notably, from the perspective of ACC design, it actually appears reasonable to have a larger $\delta_0$ if the headway setting is small as it can increase the spacing level and enhance safety.  Otherwise, the excessively small spacing could be too risky, especially in high speed.  For example, the $\tau_0=0.54s$ for car model X in the minimum headway (from consolidated data) is only one third of HDV reference.  However, if such a large $\delta_0$ is used for the entire speed range, the ACC spacing in very low speed could significantly exceed HDV traffic and that may invite surrounding vehicles to cut-in.  
%Such problems naturally result from the combination of small $\tau_0$ and large $\delta_0$. 
Therefore, \textit{we conjecture that, to accommodate the safety needs of the small headway, an ACC system tends to use a larger $\delta_0$ value for medium to high speed but ACC will switch to another $s-v$ relationship in the very low speed conditions}.  This is also consistent with the finding in \cite{shi2021empirical}.
Further research along this line is needed.

% Interestingly, our estimated $\delta_0$ values are consistent with the result in \cite{gunter2020commercially} that used another method (more discussion will follow in Section \ref{method_comparison_to_Dans}).  Moreover, the direct measurement of  $\delta_0$ from the GA experiment suggests that the large values are possible.  Further research, like the GA experiment, is desired to confirm the extrapolation for  $\delta_0$ here.  

% maybe to save this for future papers when extrapolating the results. In this case, let's not color it based on the brands. 
% In the figure, each color of the markers captures one manufactures.  For the green and blue groups, each has several car systems.  Interestingly, the green and blue groups cluster in the upper left region when under the minimum headway; i.e., very small  $\tau_0$ and large $\delta_0$. \todo{maybe to save this for future papers when extrapolating the results.} 












\noindent
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=.5\textwidth]{figures/tau0_vs_delta0.png}
\captionof{figure}{$\tau_0$ and $\delta_0$ pairs of the evaluated ACC systems}
\label{tau0_vs_delta0}
\end{minipage}



\subsection{\textbf{The fundamental diagrams}}

Based on the an estimated $s-v$ relationships, we have estimated the corresponding fundamental diagram.  Below, we will show the characteristics of capacity, jam density, and wave speed. 

% Specifically, a linear $s-v$ relationship translates to a triangular shaped fundamental diagram; i.e.,  $w= -\delta_0/\tau_0$, $k_j= 1/\delta_0$, and $Cap = u_f / (u_f \tau_0 + \delta_0) =- k_j w u_f/(u_f-w)$. Note that the capacity depends on free-flow speed $u_f$. 
% In the ACC systems tested, the highest speed is about $105km/h (65mph)$ with a small variation and thus we project the capacity based on the $s-v$ relationship by assuming that $u_f=105km/h$. 
% Here we project the capacity at $u_f=105km/h$ $(65mph)$ as it is about the higher bound of the ACC systems tested. 
Figure \ref{q_k_overall}(b) shows the $q-k$ relationships (in black lines) of the evaluated ACC systems, directly corresponding to the $s-v$ relationships in Figure \ref{q_k_overall}(a) . 
% We also add the reference of HDVs (in red dashed lines) based on NGSIM data.  Specifically, in the $s-v$ relationship, the lower/upper bound is obtained by minimum/maximum $\tau_0$ and $\delta_0$ from the observations in \cite{CHEN20121440}. In the $q-k$ relationship, the lower/upper bound is obtained by calculating the wave speed $w=-\delta_0/\tau_0$ and jam density $k=1/\delta_0$ using the maximum/minimum $\tau_0$ and $\delta_0$.


\noindent
\begin{minipage}{\linewidth}
\centering
\begin{minipage}[b]{.49\linewidth}
\centering
\small
\includegraphics[height=150pt]{figures/s-v overall.png}
\\[-6pt]
(a) s-v relationship
\end{minipage}
\begin{minipage}[b]{.49\linewidth}
\centering
\small
\includegraphics[height=150pt]{figures/q-k overall.png}
\\[-6pt]
(b) q-k relationship
\end{minipage} 
\captionof{figure}{FD of the evaluated ACC systems (colored scatters are from the consolidated data and the grey ones from the non-consolidated ones)
}
\label{q_k_overall}
\end{minipage}



Figure \ref{capacity_dist} shows the distribution of capacity for the evaluated ACC systems compared to the HDV reference (red dashed line for mean and orange dotted lines for upper and lower bounds). 
Note that the variation in the HDV capacity corresponds to the potential capacity variation due to the heterogeneity of individual HDV (potentially a holistic outcome of heterogeneity in the vehicle and the driver behavior).  %E.g., the maximum capacity in HDVs corresponds to the driver that maintains the minimum spacing ($\delta_0+\tau_0*u_f$) at $u_f$.  
Clearly, the distribution exhibits two clusters, where the larger (smaller) value group represent the capacity upper (lower) bounds of the ACC systems resulting from the minimum (maximum) headway.  One can see that the ACC systems can reach a higher capacity than HDVs. For example, the three highest capacity values are 3593$veh/h$ (H-min), 3430$veh/h$ (X-min), and 3322$veh/h$ (W-min), while the maximum possible capacity for HDVs is 3448$veh/h$. Here we use H-min to denote ACC system H under minimum headway setting. On the other hand, ACC will result in very small capacity when under the maximum headway. For example, it is 1323$veh/h$ for Model S-max, 1380$veh/h$ for C-max, and 1387$veh/h$ for X-max, which is close to the minimum possible capacity for HDV.  Clearly, when the traffic flow consists of ACC and HDVs, the roadway capacity will vary in a wide range, depending on (i) the user preference of headway setting, and (ii) the penetration rates of the various ACC systems.  Nevertheless, the upper bound (3593$veh/h$) and lower bound (1323$veh/h$) estimated from the ACC pool serve as the bounds of the mixed traffic.  

\noindent
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=.45\textwidth]{figures/capacity_dist.png}
\captionof{figure}{Capacity distribution of the evaluated ACC systems}
\label{capacity_dist}
\end{minipage}



We also examine $w$, the slope of the congestion branch on the fundamental diagram, which represents the average wave speed when ACC transitions from one equilibrium state to another. $w$ is estimated by $w=-\delta_0/\tau_0$. Figure \ref{wave_dist} shows the distribution of $w$ for the 17 evaluated ACC systems (different headway settings are separated).  On top of that, we also show the typical range of $w$ in HDV traffic (-20$km/h$ to -10$km/h$) in the literature  \citep{chen2012behavioral,laval2010mechanism,duret2011passing,chen2014periodicity} as a reference. Clearly, the $w$ value from the ACC systems varies largely (-103.8$km/h$ to -8.0$km/h$) and can be much larger than HDV traffic.  Particularly, the most negative $w$ is -103.8$km/h$ on system G-min, resulting from a small $\tau_0$ (0.61$s$) and large $\delta_0$ (17.44$m$). This fast propagating wave is a unique feature of ACC systems. It indicates  that, once a state transition occurs (e.g., a bottleneck is activated),  it can potentially be transferred to upstream in an extreme fast speed and therefore might have severer impacts (e.g., a fast-stacked queue).  Nevertheless, it should be noted that the wave speed here is calculated from equilibrium data points. The ACC non-equilibrium behaviors at state transitions are not directly captured. Further studies are being conducted to directly study the wave speed features.

% \hl{add something about implication of w here}

% Note that in the conventional HDV traffic, $\tau_0$ is the trip travel time of the shock wave (i.e., the time that the follower takes to respond to her leader's speed change).  Accordingly,  $w$ captures the wave speed in congestion.  However, in an ACC system, $\tau_0$ is the time gap used in the controller and thus $w$ may not represent the shock wave propagation speed. To retain a reasonable scope, we will investigate the  propagation of traffic state change in ACC systems in a sequential paper.  


% Notably, $w$ here is estimated from $\delta_0$ and $\tau_0$ pertaining to equilibrium traffic; i.e., it is not directly measured by tracking the propagation of traffic state change.  For the dynamics of traffic state change, later in \ref{non-equi} we will examine how ACC systems react when the leader deviates from equilibrium to decelerate and/or accelerate.



\noindent
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=.45\textwidth]{figures/wave_speed_dist.png}
\captionof{figure}{Wave speed distribution of the evaluated ACC systems}
\label{wave_dist}
\end{minipage}


We also obtain the jam density $k_j$, which is directly obtained from the estimated $\delta_0$; i.e., $k_j=1/\delta_0$. Figure \ref{jam_dist} shows the distribution of $k_j$ and a reference from HDVs estimated from NGSIM per \cite{chen2012behavioral}. One can see that the $k_j$ of ACC systems varies in a much larger range than HDVs. Moreover, a large proportion of ACC systems %(56\%) 
have a $k_j$ below the lower bound of the HDVs, %(93$veh/km$, corresponding to $\delta_0=10.74m$), 
corresponding to ACC systems with large $\delta_0$ values in Figure \ref{time-gap-jam-spacing_dist}(b).  Again, we caution that the $k_j$ is the extrapolated outcome and future tests are needed to directly measure  $\delta_0$ and thus $k_j$. 


% From the $s-v$ relationship, we obtain the corresponding jam density $k_j$ for an FD, $k_j=1/\delta_0$.  Figure \ref{jam_dist} shows the distribution of $k_j$ and a reference from HDVs estimated from NGSIM per \cite{chen2012behavioral}.  One can see that the $k_j$ of ACC systems varies in a much larger range than HDVs. Moreover, a large proportion of ACC systems (57\% ) have a $k_j$ below the lower bound of the HDVs (93$veh/km$, corresponding to $\delta_0= x$), which correspond to ACC systems with large $\delta_0$ values in Figure \ref{time-gap-jam-spacing_dist}(b).  Notably, due to the experiment setup, we do not have direct observations for vehicles at complete stop (the minimum speed in the MA Experiment is 10$m/s$ and 5$m/s$ in the Work Experiment). Therefore, the estimated $\delta_0$ is a projection from the linear $s-v$ relationship, not the actual measurement. We caution that, it is likely that the estimated $\delta_0$ (and thus $k_j$) value does not necessarily translate to the \textit{actual} jam spacing (jam density) one would observe.  Moreover, it is unclear whether the $s-v$ relationships obtained will still hold in low speed ($<$10$m/s$). Further empirical tests are needed to investigate these issues.


\noindent
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=.45\textwidth]{figures/jam_density_dist.png}
\captionof{figure}{Jam density distribution of the evaluated ACC systems}
\label{jam_dist}
\end{minipage}





% \subsection{\textbf{Discussion on spacing variation}}

% Another important feature we observe in the data is the spacing variation in a bin. Figure \ref{speed_bin}(a) shows an example of the observed $s-v$ relationship on a tested car model (Tesla Model X, maximum headway).  The recognized bins are shown as vertical transparent bars on the $s-v$ plane. Moreover, if there are more than 10 sample points in the bin, the bin is denoted in red color, otherwise it is grey. The bins with sufficient points allow us to investigate the distribution on ACC spacing under similar speed. Here, figure \ref{speed_bin} (b) and (c) shows the distribution of spacing in the two main bins (in red) of system X. One can see that the spacing is normally distributed in each bin, which is found generally hold in the bins we observed in every system.


% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \begin{minipage}[b]{.49\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=.75\textwidth]{figures/speed bins.png}
% \\[-2pt]
% (a) $s-v$ relationship
% \end{minipage}

% \begin{minipage}[b]{.49\linewidth}
% \footnotesize
% \centering
% \includegraphics[width=.75\textwidth]{figures/speed bin dist 1.png}
% \\[-2pt]
% (b) distribution of spacing between \SI{7.35}{m/s} to \SI{8.47}{m/s}
% \end{minipage} 
% \begin{minipage}[b]{.49\linewidth}
% \footnotesize
% \centering
% \includegraphics[width=.75\textwidth]{figures/speed bin dist 2.png}
% \\[-2pt]
% (c) distribution of spacing between \SI{10.85}{m/s} to \SI{11.32}{m/s}
% \end{minipage} 
% \captionof{figure}{An example of speed bin recognition and spacing distribution in the bins}
% \label{speed_bin}
% \end{minipage}



% Figure \ref{speed_bin_STD}(a) shows the relationship of the bin STD with the number of data point in the speed bin. It is found that when the number of data points is less, the STD can vary much. When the sample size is small, the distribution might not be completely measured, therefore few extreme case can significantly enlarge the variance. As the number of data points increases, the STD has a trend to converge (at around \SI{1.5}{m} to \SI{2}{m}). This result indicates that, to have a confident observation of equilibrium spacing at certain speed levels, a reasonable number of observation points is needed. It is also found that the OpenACC-AstaZero data has a consistently low variance, while the variance levels in OpenACC-ZalaZone, MA experiments, and Work experiments are higher.
% Figure \ref{speed_bin_STD}(b) shows the relationship of the bin STD with the mean bin speed. No significant pattern is found.

% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \begin{minipage}[b]{.49\linewidth}
% \footnotesize
% \centering
% \includegraphics[width=.75\textwidth]{figures/speed bin std vs sample size.png}
% \\[-2pt]
% (a) number of equilibrium samples
% \end{minipage} 
% \begin{minipage}[b]{.49\linewidth}
% \footnotesize
% \centering
% \includegraphics[width=.75\textwidth]{figures/speed bin std vs speed.png}
% \\[-2pt]
% (b) speed
% \end{minipage} 
% \captionof{figure}{The relationship of the bin standard deviation with sample size and speed}
% \label{speed_bin_STD}
% \end{minipage}


% % example trajectory of different equilibrium spacing in the same speed (high and low bound)

% The spacing variances of ACC controllers observed in the empirical data is surprising. We cautiously note that, the variances can be related to three potential sources: (i) measurement errors in the data collection process,  (ii) characteristics of ACC controllers, and (iii)  criteria for selecting equilibrium intervals.

% First, the measurement errors are not negligible in the data collection process. Specifically, it is known the MA experiments, Work experiments, and OpenACC-ZalaZone use similar GPS devices as the main data collecting source. Based on our own tests, the mean location error of the GPS device is \SI{0.89}{m}, while the method used in OpenACC-AstaZero is claimed to be more accurate with the mean location error at \SI{0.02}{m}. The accuracy difference is comparable to the extra standard deviation observed in the three GPS-based data sets (Mean bin STD - OpenACC-ZalaZone: \SI{1.43}{m}, MA experiments: \SI{1.68}{m}, Work experiments: \SI{1.36}{m}, OpenACC-AstaZero: \SI{0.58}{m}). 

% There are still a considerable level of spacing variances even after exempting the measurement error (e.g., the AstaZero data). The hardware and software (algorithm) of ACC system itself could also contribute to the spacing variances. Note that an ACC system rely on sensors to provide the distance and speed measurement of leader. This process can introduce errors due to sensor noises. When the incorrect inputs are given to the ACC algorithm, the system can mis-comprehend and reach equilibrium when it should not be. On the other hand, as the manufacturers are aware of the sensor noises, ACC design usually considers some buffer styles that prevent the controller being too sensitive to noises. For example, []. This might also lead to an equilibrium 'zone' in the controller, i.e., variances on equilibrium spacing.

% Finally, we note that the criteria for selecting equilibrium intervals can play a role in the variances. Particularly, in real-world traffic, due to the changing environment (e.g., aerodynamic, gradient, pavement condition), vehicle controllers have to adjust the speed dynamically, i.e., there is no \textit{strict} equilibrium (i.e., zero speed and spacing change) in the traffic. Therefore, we have to allow certain criteria to recognize equilibrium intervals from the data, which will inevitably introduce some variances. Nevertheless, we have tried a stricter bound for selecting equilibrium intervals (\SI{0.11}{m/s} for speed and \SI{0.25}{m} for spacing). It is found the equilibrium sample size will squeeze, but the spacing variances still exist when multiple samples are observed in a bin. 

% % Moreover, in relatively rare but still existing conditions, the location error can be even higher (\SI{2.30}{m} for the 90th percentile of error distribution). This could contribute to the cases where the spacing range at a certain speed is large range.




% To further examine the the spacing (flow) variation, we adopt the $\eta$ framework per \cite{chen2012behavioral}, which is an extension of Newell's simplified CF model \citep{newell2002simplified}. In congestion Newell's model predicts that the trajectory of a follower is identical to that of its leader except for a translation in space-time; we call this trajectory ``Newell trajectory''; see Fig.\ref{eta_framework}. Specifically, $\eta$ is the indicator that describes the deviation of the follower with respect to the Newell trajectory (i.e. average equilibrium in our context), defined as:
% \begin{equation}
%     \eta_{i}(t) = \tau_{i}(t)/\tau
% \end{equation}
% where $\tau_{i}(t)$ is the actual wave travel time of vehicle $i$ at time point $t$ and $\tau$ is the average equilibrium wave travel time. Note that $\tau$ is equivalent to the time gap value $\tau_0$ of an ACC controller. Here $\tau_0$ is an constant taken from the linear estimation results. $\tau_{i}(t)$ is measured along an constant wave speed $w = -\delta_0/\tau_0$. If $\eta<1$ then the vehicle is in front of the Newell trajectory and therefore driving more aggressively than the average; similarly, $\eta>1$ implies a more timid driving behavior.


% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \includegraphics[width=.45\textwidth]{figures/eta_measurement.png}
% \captionof{figure}{$\eta$ framework \citep{chen2012behavioral}}
% \label{eta_framework}
% \end{minipage}

% Particularly, we show the long-term $\eta$ evolution of three systems in their minimum headway setting (X-min, Y-min, Z-min), which have been tested in an extensive time scale, in Fig.\ref{long_term_eta_measurement} (a)(b)(c). For each system, $\eta$ is measured along the wave $w = -\delta_0/\tau_0$ calculated based on the estimated $\delta_0$ and $\tau_0$ of them. In the figure, The grey areas mark the recognized equilibrium intervals. For each interval, we measure the mean $\eta$ level during it, denoted as $\eta_0$. Fig.\ref{long_term_eta_measurement}(d)(e)(f) show the corresponding $\eta_0$ values of the three systems in the temporal sequential order.

% Clearly, a small variation of $\eta_0$ (smaller than $\pm$0.1) is seen on all three ACC systems.  Moreover, a Ljung-Box test \citep{ljung1978measure} (with time lag = 1) shows that the data points are independent and identically distributed over time, suggesting that the $\eta_0$ fluctuation is random. Particularly, we conduct a paired t-test on the 12 $\eta_0$ pairs of X-min before and after a driving cycle (Y-min and Z-min are not tested as the sample size is small) and find that there is no significant difference (p-value = 0.55). Thus, the results here suggest that the variation in the $s-v$ relationship, and thus the flow fluctuation pertaining to the free-flow speed, is inherent to the controller.  



% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \begin{minipage}[b]{\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=.85\textwidth]{figures/long term eta tesla 3.png}
% \\[-6pt]
% (a) long term $\eta$ evolution (X-min)
% \end{minipage}
% \begin{minipage}[b]{\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=.85\textwidth]{figures/long term eta civic.png}
% \\[-6pt]
% (b) long term $\eta$ evolution (Y-min)
% \end{minipage}
% \begin{minipage}[b]{\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=.85\textwidth]{figures/long term eta prius.png}
% \\[-6pt]
% (c) long term $\eta$ evolution (Z-min)
% \end{minipage}

% \begin{minipage}{.32\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/eta_time_model3.png}

% (d) $\eta_0$ values over time (X-min)
% \end{minipage}
% \begin{minipage}{.32\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/eta_time_civic.png}

% (e) $\eta_0$ values over time (Y-min)
% \end{minipage}
% \begin{minipage}{.32\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/eta_time_prius.png}

% (f) $\eta_0$ values over time (Z-min)
% \end{minipage}
% \captionof{figure}{long term $\eta$ evolution of ACC systems}
% \label{long_term_eta_measurement}
% \end{minipage}


==> sections/old/6_Discussion.tex <==
\section{\textbf{Discussions}}\label{Sec discussion}
In this session, we will show that our direct approach to estimate $s-v$ (and thus FD) of ACC systems produces consistent results with the prevalent method in the literature - the controller calibration, which further validates our results.  Additionally, we will investigate the measurement variance observed in our analysis, which inevitably occurs in direct measurement but would be hidden if the controller calibration approach is used. 

\subsection{\textbf{Methods to estimate $s-v$ relationships}}\label{method_comparison_to_Dans}

% \todo[inline]{
% - introduce the concept of CI. 
% - in general, estimation from Gunter et al. falls within the CI of our estimation, suggesting that the two methods are consistent. This is also reflected by the small difference in tau and delta. 
% - caution: Gunter et al. also assumes a single equilibrium relationship, which is essentially the same spirit with our method.  
% }

In this paper, we have directly measured ($s$, $v$) in equilibrium periods and use that to estimate the $s-v$ relationships, and thus the FDs, of an ACC system.  Yet, the controller calibration approach is more commonly used in the literature, which often uses all data, including equilibrium and non-equilibrium conditions, to calibrate a controller.  For example, \citep{gunter2020commercially, gunter2019model} calibrated a general optimal velocity relative velocity (OVRV) car-following model, which essentially yields the same $s-v$ relationship as Equation (\ref{linear SV}) for equilibrium conditions. Similar practice was applied in \cite{shi2021empirical}. 
Here we are interested in the results from the two different methods.  To test that, we compare our results with those reported in \cite{gunter2020commercially, gunter2019model} using the Work Experiment data.    
% results from the Work Experiment data.  
% Particularly, \cite{gunter2020commercially, gunter2019model} have reported the fitted coefficient and intercept terms (i.e., $\tau_0$ and $\delta_0$ in this paper) for ACC system A-H. As we use the same data but a different method for the estimation of $s-v$ relationships, we are interested on whether the two methods will lead to comparable results. 
We adopt the concept of confidence intervals (CI) for linear regressions \citep{fisher1956statistical} to compare the estimation results with the two methods. Figure \ref{dan_comparision} shows one example of the comparison (system D, maximum headway). One can see the differences of $\tau_0$ and $\delta_0$ are small between the two methods. Moreover, the estimated $s-v$ from OVRV model (red dashed line) falls within the 95\% CI (blue curves) of the linear regression from equilibrium data. 

Among the 17 ACC systems (different headway setting is treated as a different system), eight of them have the OVRV results completely within the 95\% CI from equilibrium data.  The other have some parts of the OVRV estimation outside the 95\% CI but mostly are within the CI. The plots and estimated results are provided in Appendix \ref{dan_comparison_complete}. %\todo{are we goign to provide that?} 
%In none of the cases, the two estimation results are totally off. 
The results suggest that the two methods are consistent in general.  This is not surprising as the method used in \cite{gunter2020commercially,gunter2019model} essentially assume a single linear $s-v$ for the tested data, the same spirit with our method. 

\noindent
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=.45\textwidth]{figures/Dan_comparison.png}
\captionof{figure}{Comparison of the estimation results from the equilibrium data and OVRV model (D-max)}
\label{dan_comparision}
\end{minipage}


%We do caution that, neither methods would not be able to capture the potential piece-wise linearity or non-linearity in the ACC controller behaviors, if there is any. Suck behavior transition needs further investigation in the future.



\subsection{\textbf{Spacing variation}}\label{spacing_variation}
In our analysis of the equilibrium points, we observe that there may exist significant spacing in some speed bins, translating to significant flow variation at a given speed. Figure \ref{speed_bin}(a) shows an example of the observed $s-v$ relationship on Tesla Model S with maximum headway. The recognized bins are shown as vertical transparent bars on the $s-v$ plane. Moreover, if there are more than 10 sample points in the bin, the bin is denoted in red color. Otherwise it is grey. The bins with sufficient points allow us to investigate the distribution on ACC spacing under similar speed. Here, figure \ref{speed_bin} (b) and (c) shows the distribution of spacing in the two main bins (in red) in figure \ref{speed_bin} (a). One can see that the spacing appears normally distributed in each bin.  We find that generally holds in the bins we observed in every system.


\noindent
\begin{minipage}{\linewidth}
\centering
\begin{minipage}[b]{.49\linewidth}
\centering
\footnotesize
\includegraphics[width=.75\textwidth]{figures/speed bins.png}
\\[-2pt]
(a) $s-v$ relationship
\end{minipage}

\begin{minipage}[b]{.49\linewidth}
\footnotesize
\centering
\includegraphics[width=.75\textwidth]{figures/speed bin dist 1.png}
\\[-2pt]
(b) distribution of spacing between \SI{7.68}{m/s} to \SI{8.86}{m/s}
\end{minipage} 
\begin{minipage}[b]{.49\linewidth}
\footnotesize
\centering
\includegraphics[width=.75\textwidth]{figures/speed bin dist 2.png}
\\[-2pt]
(c) distribution of spacing between \SI{10.85}{m/s} to \SI{11.21}{m/s}
\end{minipage} 
\captionof{figure}{An example of speed bin recognition and spacing distribution in the bins}
\label{speed_bin}
\end{minipage}



A closer look of the spacing variation shows that the standard deviation can be large ($>3m$) if the number of data points is small, but converges to a reasonable level (around \SI{1.5}{m}) as sample size increases (40 points or more); see Figure \ref{speed_bin_STD}.  It is also found that the OpenACC-AstaZero data (red points) has a consistently lower variance than the other data sources.  This is likely because AstaZero has a measurement system with larger accuracy (mean location error was claimed to be \SI{0.02}{m} \cite{makridis2021openacc}).  Note that 
the MA experiments, Work experiments, OpenACC-ZalaZone, and GA experiment used similar GPS devices as the main data collection tool and have similar error ranges (the mean ranges from \SI{1.36}{m} to \SI{1.68}{m}). 




% Figure \ref{speed_bin_STD}(a) shows the relationship of the bin standard deviation with the number of data point in the speed bin. One can see that the standard deviation can be large (larger than 3m) if the number of data points is small.  But as the number increases, the standard deviation converges to a reasonable level (around \SI{1.5}{m} to \SI{2}{m}). This result indicates that, to have a confident observation of equilibrium spacing at a speed level, a reasonable number of observation points is needed. It is also found that the OpenACC-AstaZero data (red points) has a consistently lower variance than the other data sources.  This is likely because AstaZero has a measurement system with larger accuracy (mean location error was claimed to be \SI{0.02}{m} \cite{makridis2021openacc}).  Note that 
% the MA experiments, Work experiments, OpenACC-ZalaZone, and GA experiment used similar GPS devices as the main data collection tool and have similar error ranges (the mean ranges from \SI{1.36}{m} to \SI{1.68}{m}). Our tests show that, the location error from two GPS devices (placed side by side) has a mean of \SI{0.89}{m}. %The accuracy difference is comparable to the extra standard deviation observed in the three GPS-based data sets (Mean bin STD - OpenACC-ZalaZone: \SI{1.43}{m}, MA experiments: \SI{1.68}{m}, Work experiments: \SI{1.36}{m}, OpenACC-AstaZero: \SI{0.58}{m}). 
% The results here suggests that preferably ACC field tests should use highly accurate measurement systems and have sufficient repetitions.  

\noindent
\begin{minipage}{\linewidth}
\centering
\begin{minipage}[b]{.49\linewidth}
\footnotesize
\centering
\includegraphics[width=.75\textwidth]{figures/speed bin std vs sample size.png}
\\[-2pt]
% (a) number of equilibrium samples
\end{minipage} 
% \begin{minipage}[b]{.49\linewidth}
% \footnotesize
% \centering
% \includegraphics[width=.75\textwidth]{figures/speed bin std vs speed.png}
% \\[-2pt]
% (b) speed
% \end{minipage} 
\captionof{figure}{The relationship of the bin standard deviation with sample size and speed}
\label{speed_bin_STD}
\end{minipage}


% example trajectory of different equilibrium spacing in the same speed (high and low bound)

We find that spacing variation is still observed even we impose stricter criteria on the equilibrium conditions (e.g., \SI{0.11}{m/s} for speed variation and \SI{0.25}{m} for spacing variation) and sample size from the highly accurate AstaZero data.  Two factors can contribute to that.  Firstly, note that in real-world traffic, due to the changing environment (e.g., aerodynamic, gradient, pavement condition), it is extremely difficult, if possible at all, for a vehicle to stay in the absolute equilibrium condition for a significant period of time.  Thus, the equilibrium intervals measured will almost inevitably have some variation in the traffic states (stricter criteria will help to reduce the variation to a certain extent but couldn't fully eliminate that).  Additionally, notice that the ACC systems rely on sensors (mostly radar and/or camera) to provide the distance and speed measurement of leader, which have measurement errors.  Such errors could result in mis-perception in ACC (e.g., its speed doesn't change even there is a spacing deviation from equilibrium) and thus contribute to the spacing variation. 

% First, the measurement errors are not negligible in the data collection process. Specifically, it is known the MA experiments, Work experiments, and OpenACC-ZalaZone use similar GPS devices as the main data collecting source. Based on our own tests, the mean location error of the GPS device is \SI{0.89}{m}, while the method used in OpenACC-AstaZero is claimed to be more accurate with the mean location error at \SI{0.02}{m}. The accuracy difference is comparable to the extra standard deviation observed in the three GPS-based data sets (Mean bin STD - OpenACC-ZalaZone: \SI{1.43}{m}, MA experiments: \SI{1.68}{m}, Work experiments: \SI{1.36}{m}, OpenACC-AstaZero: \SI{0.58}{m}). 

% There are still a considerable level of spacing variances even after exempting the measurement error (e.g., the AstaZero data). 

% The hardware and software (algorithm) of ACC system itself could also contribute to the spacing variances. Note that an ACC system rely on sensors to provide the distance and speed measurement of leader. This process can introduce errors due to sensor noises. When the incorrect inputs are given to the ACC algorithm, the system can mis-comprehend and reach equilibrium when it should not be. \hl{On the other hand, as the manufacturers are aware of the sensor noises, ACC design usually considers some buffer styles that prevent the controller being too sensitive to noises. For example, []. This might also lead to an equilibrium 'zone' in the controller, i.e., variances on equilibrium spacing.}\todo{do we have any evidence on that?}

% Finally, we note that the criteria for selecting equilibrium intervals can play a role in the variances. Particularly, in real-world traffic, due to the changing environment (e.g., aerodynamic, gradient, pavement condition), vehicle controllers have to adjust the speed dynamically, i.e., there is no \textit{strict} equilibrium (i.e., zero speed and spacing change) in the traffic. Therefore, we have to allow certain criteria to recognize equilibrium intervals from the data, which will inevitably introduce some variances. Nevertheless, we have tried a stricter bound for selecting equilibrium intervals (\SI{0.11}{m/s} for speed and \SI{0.25}{m} for spacing). It is found the equilibrium sample size will squeeze, but the spacing variances still exist when multiple samples are observed in a bin. 

% Moreover, in relatively rare but still existing conditions, the location error can be even higher (\SI{2.30}{m} for the 90th percentile of error distribution). This could contribute to the cases where the spacing range at a certain speed is large range.


% \todo{I feel the part below is not very critical. We could probably remove it}
% {\color{blue}

% To further examine the the spacing (flow) variation, we adopt the $\eta$ framework per \cite{chen2012behavioral}, which is an extension of Newell's simplified CF model \citep{newell2002simplified}. In congestion Newell's model predicts that the trajectory of a follower is identical to that of its leader except for a translation in space-time; we call this trajectory ``Newell trajectory''; see Fig.\ref{eta_framework}. Specifically, $\eta$ is the indicator that describes the deviation of the follower with respect to the Newell trajectory (i.e. average equilibrium in our context), defined as:
% \begin{equation}
%     \eta_{i}(t) = \tau_{i}(t)/\tau
% \end{equation}
% where $\tau_{i}(t)$ is the actual wave travel time of vehicle $i$ at time point $t$ and $\tau$ is the average equilibrium wave travel time. Note that $\tau$ is equivalent to the time gap value $\tau_0$ of an ACC controller. Here $\tau_0$ is an constant taken from the linear estimation results. $\tau_{i}(t)$ is measured along an constant wave speed $w = -\delta_0/\tau_0$. If $\eta<1$ then the vehicle is in front of the Newell trajectory and therefore driving more aggressively than the average; similarly, $\eta>1$ implies a more timid driving behavior.


% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \includegraphics[width=.45\textwidth]{figures/eta_measurement.png}
% \captionof{figure}{$\eta$ framework \citep{chen2012behavioral}}
% \label{eta_framework}
% \end{minipage}

% Particularly, we show the long-term $\eta$ evolution of three systems in their minimum headway setting (X-min, Y-min, Z-min), which have been tested in an extensive time scale, in Fig.\ref{long_term_eta_measurement} (a)(b)(c). For each system, $\eta$ is measured along the wave $w = -\delta_0/\tau_0$ calculated based on the estimated $\delta_0$ and $\tau_0$ of them. In the figure, The grey areas mark the recognized equilibrium intervals. For each interval, we measure the mean $\eta$ level during it, denoted as $\eta_0$. Fig.\ref{long_term_eta_measurement}(d)(e)(f) show the corresponding $\eta_0$ values of the three systems in the temporal sequential order.

% Clearly, a small variation of $\eta_0$ (smaller than $\pm$0.1) is seen on all three ACC systems.  Moreover, a Ljung-Box test \citep{ljung1978measure} (with time lag = 1) shows that the data points are independent and identically distributed over time, suggesting that the $\eta_0$ fluctuation is random. Particularly, we conduct a paired t-test on the 12 $\eta_0$ pairs of X-min before and after a driving cycle (Y-min and Z-min are not tested as the sample size is small) and find that there is no significant difference (p-value = 0.55). Thus, the results here suggest that the variation in the $s-v$ relationship, and thus the flow fluctuation pertaining to the free-flow speed, is inherent to the controller.  



% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \begin{minipage}[b]{\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=.85\textwidth]{figures/long term eta tesla 3.png}
% \\[-6pt]
% (a) long term $\eta$ evolution (X-min)
% \end{minipage}
% \begin{minipage}[b]{\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=.85\textwidth]{figures/long term eta civic.png}
% \\[-6pt]
% (b) long term $\eta$ evolution (Y-min)
% \end{minipage}
% \begin{minipage}[b]{\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=.85\textwidth]{figures/long term eta prius.png}
% \\[-6pt]
% (c) long term $\eta$ evolution (Z-min)
% \end{minipage}

% \begin{minipage}{.32\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/eta_time_model3.png}

% (d) $\eta_0$ values over time (X-min)
% \end{minipage}
% \begin{minipage}{.32\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/eta_time_civic.png}

% (e) $\eta_0$ values over time (Y-min)
% \end{minipage}
% \begin{minipage}{.32\linewidth}
% \centering
% \footnotesize
% \includegraphics[width=\textwidth]{figures/eta_time_prius.png}

% (f) $\eta_0$ values over time (Z-min)
% \end{minipage}
% \captionof{figure}{long term $\eta$ evolution of ACC systems}
% \label{long_term_eta_measurement}
% \end{minipage}

% }


% \subsection{\textbf{Speed ranges for the $s-v$ relationships}}
% None of the experiments in the literature has tested ACC in the full speed ranges as the experiments were designed for different purposes. Figure \ref{speed_range} shows the tested speed range of the car models from the four experiments (see the grey bar) and the observed equilibrium cases (see the red slots). The car models are only tested in a partial speed range and the equilibrium cases only cover a set of discrete speed levels. While linear approximation seems a good fit for the tested ranges, the estimated $s-v$ relationship may change outside the ranges.  It's also possible that the overall relationship is non-linear but linear is a reasonable approximation for a certain speed range.  Future research is need to complete the coverage, especially the low speed ranges.  

% \noindent
% \begin{minipage}{\linewidth}
% \centering
% \includegraphics[width=.6\textwidth]{figures/speed range.png}
% \captionof{figure}{Observed equilibrium speed %(grey bar indicates the overall range, red slots indicate the speed bins with observed equilibrium cases)
% }
% \label{speed_range}
% \end{minipage}


